RKHS-BA: A Robust Correspondence-Free Multi-View Registration Framework with Semantic Point Clouds

This work reports a novel multi-frame Bundle Adjustment (BA) framework called RKHS-BA. It uses continuous landmark representations that encode RGB-D/LiDAR and semantic observations in a Reproducing Kernel Hilbert Space (RKHS). With a correspondence-free pose graph formulation, the proposed system constructs a loss function that achieves more generalized convergence than classical point-wise convergence. We demonstrate its applications in multi-view point cloud registration, sliding-window odometry, and global LiDAR mapping on simulated and real data. It shows highly robust pose estimations in extremely noisy scenes and exhibits strong generalization with various types of semantic inputs. The open source implementation is released in https://github.com/UMich-CURLY/RKHS_BA.

==> frontend.tex <==
\section{Visual Odometry Frontend}
\label{sec:frontend}

\subsection{Hierachical Semantic Tracking}
\label{subsec:tracking}
\jw{TODO: framework structure is needed.}Sequential frame to frame tracking provides an initial pose for the newly incoming frame. It is a special case of \eqref{eq:inner_product_actual} which has only two frames, but still uses full hierachical semantic information. We use gradient ascent in the optimization, while the only variable is their relative pose. Detailed optimization steps are in ~\cite{clarkmaani20}.

\subsection{Keyframe Selection}
\label{subsec:keyframe}
A \textit{keyframe} is defined as follows: a) The first two frames are always keyframes. b) When the new frame does not has a large \textit{overlap} with the last keyframe, it is also a new keyframe. To measure the overlap, the tracking pose is firstly converted to the relative pose between the last keyframe and the new incoming frame. Then the amount of overlap is calculated based on the $\textit{cosine}$ alignment measure proposed in SemanticCVO~\cite{Zhang2021scvo}, defined as
\begin{equation}
\label{eq:overlap}
 \cos(\theta) = \dfrac{\langle f_X,f_{\Tb Z}\rangle_{\Hcal}}{\lVert f_X \rVert \cdot \lVert f_{\Tb Z} \rVert} .
% = \dfrac{1}{{\lVert f_X \rVert \cdot \lVert f_Z \rVert}} \sum_{\substack{x_i\in X, z_j\in Z}} c_{ij} \cdot k(x_i,z_j) .
\end{equation}
where the two input point clouds $X, TZ$ are the same ones used in tracking and $T$ is the relative pose. \ray{TODO: add keyframe selection visualization when the robot does not move}

\begin{figure*}[t]
 \includegraphics[width=\columnwidth]{figures/Keyframes.png}
 %\caption{Cosine alignment value of a keyframe matched against following non-keyframes, where the steady motion is from Abandonedfactory_night/Easy/P001 frame 324, and the rapid motion is from Abandonedfactory/Hard/P001 frame 237} 
 \label{fig:stereo_indicator}
 % \squeezeup
\end{figure*}

\subsection{Keyframe's keypoint selection}
\textit{Keypoints} are point candidates from the keyframes for the backend window optimization. We implement a sparse voxel grid to downsample the full input point cloud, while every voxel might contain one or more points. A single point will be sampled from each voxel. In this way, the keypoints are evenly distributed in the 3D space. Also, edge points and surface points are selected seperately with voxel fitlers of different sizes. As shown in Figure \ray{TODO}, in scenes with less corner features or with a lot of repetitive patterns, enough points would still be preserved for the backend. \ray{TODO: Figure: projected pixel selection results after Voxel grid downsampling, on normal and featureless areas.}

\subsection{Keypoint Filering}
\label{subsec:depth_filtering} 
%We use a depth filtering to filter the noisy raw input point cloud of the keyframes. 
Keypoint filtering removes noisy raw input points or outlier points from keyframes. Specifically, for the latest keyframe, we run the data association function~\eqref{eq:double_sum} between its own keypoints and all sequential non-keyframes full point cloud, based on the relative transformations from tracking. As long as a keypoint has a soft correspondence in the subsequent non-keyframes, it is considered as an inlier, which will be used in the later stage bundle adjustment. \ray{picture: depth fitler of sequential frames} 



% During the alignment, We keep track of the indicator value in our alignment step. If $i_{\theta}$ stabilized, it means 
% \cel{TODO: write about how we use it. It is described in following section but not clear.}
% value doesn't matter, we use ratio

%\section{Talk about sensors RB-D, Stereo, LIDAR}

%\subsection{Optimization}
%We perform gradient ascent over $SE(3)$ on the inner product in~\eqref{eq:double_sum}. The flow and step size expressions are in the same forms as ~\cite{MGhaffari-RSS-19}. During the iterative optimization, the alignment indicator in~\ref{subsec:indicator} can guide the lengthscale update. When the lengthscale is large, each point is associated with farther points, which provides the point cloud function a global perspective. When the lengthscale is small, each point is only connected to its closest neighbors, resulting in local attention for the registration. For a single registration process, we use larger lengthscales at early iterations. Every time the alignment indicator value at the current lengthscale stabilizes, we decay the lengthscale by a fixed percent.% until it reaches a predefined minimum value. 
%This mechanism is inspired by the deterministic annealing process in some GMM-based registration methods~\cite{chui2000mpm,granger2002multiemicp,gold1998softassign}, which perform a fixed lengthscale decay every few iterations. 

%\subsection{Depth Filtering for local keyframes}
%Each keyframe's points' depth values are refined by the coming non-keyframes. After tracking, each point, denoted as $x_i$, in the last keyframe has a set of corresponding points from the latest frame, denoted as $\{y_j^{(i)}\}$. The correspondences do not need extra computation, as they are an intermediate result from the inner product calculation during tracking. A linear regression is performed to regress this point's depth from its correspondence points. If a point from the keyframe does not have any coorespondence after multiple depth filtering , it would be classified as an \textit{outlier} and would not be added to the keyframe's local map.

==> map.tex <==
\section{Hierachical Semantic Covisibility Map}
In practice, instead of solving ~\eqref{eq:irls} for all frames,  we choose a sliding window of frames for efficiency concerns. Sliding window bundle adjustments have been successfully applied in many SLAM frameworks \citet{strasdat2011double}\citet{DSO}. Similar to \citet{mur2017orbslam2}\citet{zubizarreta2020dsm}, the sliding window consists both a temporal window and a covisible window. Temporal window contains the recent few keyframes and are densely connected. Covisible maps captures local loop closures and has be demonstrated to help the localization performance \citet{mur2015orb}\citet{zubizarreta2020dsm}.

\subsection{Covisibility Map Construction}
  %The local window not only contains the latest few time-correlated keyframes, but includes the \textit{covisible} frames that share the view of the local map as well. 
We use a global sparse voxel map to record which keyframes have observe this location, similar to \citet{muglikar2020voxel}. Specifically, for each point in the latest keyframe, with its current estimate of depth, we attach it to a nearby voxel by coordinate hashing. 

Furthermore, we can build a covisbility pose graph \citet{mur2017orbslam2}. An edge between two frames in the covisibility pose graph indicates that they share a view of the map.  By traversing through all points in this  keyframe, we obtain all the voxels the keyframe has observed. Then, for each voxel, we trace back the past keyframes which have points in the same voxel. If a past keyframe share multiple voxels with the last keyframe, they are connected in the covisibility graph. % Each time after backend's bundle adjustment, the keyframes' poses and points are updated. The voxels that contains these map points are updated correspondingly.  

	
\subsection{Covisible Map Query}
During backend's window optimization, for each keypoint in the temporal windows, we perform 3D ray-casting, until it hit a non-empty voxel. A single point from non-temporal keyframes is randomly sampled from this voxel. In this way, we are able to construct a local covisible map within a bounded time. The covisible point will be transformed into the frame of the first temporal frame in the active window and will be held fixed as an anchor during the backend optimization.
	
\subsection{Map Update}
After window bundle adjustment, the temporal frames' poses change, along with all the keypoints attached to them. We traverse through all the keypoints in the temporal frames and update the voxels they belong to so as to make the voxel map consistent.
